Approximate Bayesian Computation for an Explicit-Duration Hidden Markov Model of COVID-19 Hospital Trajectories

We address the problem of modeling constrained hospital resources in the midst of the COVID-19 pandemic in order to inform decision-makers of future demand and assess the societal value of possible interventions. For broad applicability, we focus on the common yet challenging scenario where patient-level data for a region of interest are not available. Instead, given daily admissions counts, we model aggregated counts of observed resource use, such as the number of patients in the general ward, in the intensive care unit, or on a ventilator. In order to explain how individual patient trajectories produce these counts, we propose an aggregate count explicit-duration hidden Markov model, nicknamed the ACED-HMM, with an interpretable, compact parameterization. We develop an Approximate Bayesian Computation approach that draws samples from the posterior distribution over the model's transition and duration parameters given aggregate counts from a specific location, thus adapting the model to a region or individual hospital site of interest. Samples from this posterior can then be used to produce future forecasts of any counts of interest. Using data from the United States and the United Kingdom, we show our mechanistic approach provides competitive probabilistic forecasts for the future even as the dynamics of the pandemic shift. Furthermore, we show how our model provides insight about recovery probabilities or length of stay distributions, and we suggest its potential to answer challenging what-if questions about the societal value of possible interventions.

==> tab_mae_compare_oldversion.tex <==
\newcommand{\intervalname}{2.5-97.5\% interval on MAE}
\newcommand{\ihmeintervalname}{MAE of lower - MAE of upper}
%%%%% Table: Error metrics for US
\begin{table}[!t]
\centering
\resizebox{\textwidth}{!}{%
\texttt{
\begin{tabular}{c|r |r r|r r|r r|r r| }
  & 
    & $\GG$ & \textnormal{\bf InGeneralWard} 
    & $\II + \VV$ & \textnormal{\bf InICU }
    %& $\II$ & \textnormal{\bf OffVentInICU}
    & $\VV$ & \textnormal{\bf OnVentInICU }
    & $\XX$ \textbf{sm.} & \textnormal{\bf Death}  \\ 
  & \textnormal{\bf Method}
    & MAE~ & lower - upper~
    %& MAE~ & lower - upper
    & MAE~ & lower - upper
    & MAE~ & lower - upper
    & MAE~ & lower - upper
\\  
 \hline
 \hline
 \multirow{5}{*}{MA}
  & ACED-HMM + ABC
                &  65.0~ & ~61.5 - ~~68.9  
                &  15.7~~& ~14.5 - ~16.9 
                %&  29.0~ & 27.5 - ~30.6 
                &  34.0~~& ~32.6 - ~35.7
                & ~8.0~ &   7.8 - ~8.3~~\\
  & ACED-HMM + Prior
                & 868.6~ & 779.6 - ~945.8  
                & 293.6~~&272.6 - 313.3  
                %& 291.3~ &273.5 - 309.1 
                & 119.6~~& 113.8 - 124.8
                &  40.7~ &  39.1 - 42.2~~\\                
  & AR-Poisson
                & 498.0~ & 438.3 - ~553.6  
                & 162.2~~&148.6 - 173.5  
                %&  35.5~ &~28.3 - ~43.4 
                & 128.3~~& 118.5 - 138.6
                &  34.8~ &  28.4 - 42.0~~\\    
  & IHME
                &1066.1~ & *543.4 - 1754.9 
                & 104.0~~& *15.6 - 257.9  
                %&  81.6~ & *30.0 - 151.4 
                &  25.7~~&  *41.4 - 106.5
                & 21.6~ &  *8.7 - 49.7~~\\                
  \cline{2-10}
  & Mean Test $y$
  				& 1141.6~ &                
  				& 392.5~~&               
  				%& 143.4~~&              
  				&  249.1~ &              
  				& 66.5~ & \\ 
 \cline{2-10}
 \hline
 \hline
 \multirow{3}{*}{SD}
  & ACED-HMM + ABC
                &   9.2~ &   8.5 - ~~10.1  
                &   4.5~ & ~4.3 - ~~4.8  
                %&  4.8~ &  4.7 - ~~5.0 
                &  4.8~ &  4.5 - ~~5.1 
                & ~2.8~ &  2.7 -~~2.9~ \\ 
  & IHME 
                &  71.8~ &   *6.6 - ~166.4 
                &  17.7~ & *4.2 - ~46.0  
                %& 12.6~ & *4.4 - ~25.4 
                &  5.9~ & *6.3 - ~20.6 
                & ~2.5~ & *3.6 -~~5.0~ \\ 
 \cline{2-10}
  & Mean Test $y$
  				& 102.5~ & 				  
  				& 34.9~  & 			   
  				%& 11.3~ & 				
  				& 23.6~ &  		      
  				& 7.8~  & \\
  \cline{2-10}
 \hline
 \hline
 \multirow{3}{*}{UT}
  & ACED-HMM + ABC
                &  20.8~ &  20.2 - ~~21.3 
                &  18.2~ & 17.4 - ~19.2  
                %& NA     &             
                &  NA~   &            
                & ~2.4~ &  2.3 -~~2.5~ \\
  & IHME
                & 332.9~ &*142.6 - ~578.4 
                & 105.0~ &*35.7 - 213.9  
                %& NA     &             
                &  NA~   &             
                & ~7.4~ & *2.7 -~15.7~ \\            
  \cline{2-10}
  & Mean Test $y$ 
  				& 272.9~ &               
  				& 164.3~ &               
  				%& NA     &             
  				& NA~    &             
  				& 11.7~ & \\ 
\end{tabular}}}
%\resizebox{\textwidth}{!}{%
%\begin{tabular}{ |c|r r |r|r|r|r|r| }
% \hline
%  & & & $\GG$  & $\II$ & $\VV$ & $\II + \VV$ & $\XX$ \textbf{sm.} \\ 
% \hline
% \hline
% \multirow{5}{*}{SD} & & Mean of True Counts & 102.5 & 11.3 & 23.6 & 34.9 & 7.8 \\
%  \cline{2-8}
%  &  \multirow{2}{*}{MAE} & ACED-HMM + ABC & 9.2 & 4.8 & 4.8 & 4.5 & 2.8 \\ 
%  & &  IHME & 71.8 & 12.6 & 5.9 & 17.7 & 2.5 \\ 
%  \cline{2-8}
%  &  \intervalname & ACED-HMM + ABC & 8.5 - 10.1 & 4.7 - 5.0 & 4.5 - 5.1 & 4.3 - 4.8 & 2.7 - 2.9 \\
%  \cline{2-8}
%  & \ihmeintervalname & IHME & 6.6 - 166.4 & 4.4 - 25.4 & 6.3 - 20.6 & 4.2 - 46.0 & 3.6 - 5.0 \\
% \hline
% \hline
% \multirow{5}{*}{UT} & & Mean of True Counts & 272.9 & NA & NA & 164.3 & 11.7 \\ 
%  \cline{2-8}
%  & \multirow{2}{*}{MAE} & ACED-HMM + ABC & 20.8 & NA & NA & 18.2 & 2.4 \\ 
%  &   & IHME & 332.9 & NA & NA & 105.0 & 7.4 \\ 
%  \cline{2-8}
%  & \intervalname & ACED-HMM + ABC & 20.2 - 21.3 & NA & NA & 17.4 - 19.2 & 2.3 - 2.5 \\
%  \cline{2-8}
%  & \ihmeintervalname & IHME &  142.6 - 578.4 & NA & NA & 35.7 - 213.9 & 2.7 - 15.7 \\
% \hline
% \hline
% \multirow{9}{*}{MA} & &  Mean of True Counts & 1141.6 & 143.4 & 249.1 & 392.5 & 66.5 \\ 
%  \cline{2-8}
%  & \multirow{4}{*}{MAE}  
%  &  AR-Poisson & 498.0 & 35.5 & 128.3 & 162.2 & 34.8 \\ 
%  &   & ACED-HMM + Prior & 868.6 & 291.3 & 119.6 & 293.6 & 40.7 \\ 
%  &   & ACED-HMM + ABC & 65.0 & 29.0 & 34.0 & 15.7 & 8.0 \\ 
%  &   & IHME & 1066.1 & 81.6 & 25.7 & 104.0 & 21.6 \\ 
%  \cline{2-8}
%  &  \multirow{3}{*}{\intervalname} & AR-Poisson & 438.3 - 553.6 & ~28.3 - ~43.4 & 118.5 - 138.6 & 148.6 - 173.5 & ~28.4 - ~42.0 \\
%  &  & ACED-HMM + Prior & 779.6 - 945.8 & 273.5 - 309.1 & 113.8 - 124.8 & 272.6 - 313.3 & ~39.1 - ~42.2 \\
%  &  & ACED-HMM + ABC & ~61.5 - ~68.9 & 27.5 - ~30.6 & ~32.6 - 35.7 & ~14.5 - ~16.9 & ~~7.8 - ~~8.3 \\
%  \cline{2-8}
%  & \ihmeintervalname & IHME & 543.4 - 1754.9 & 30.0 - 151.4 & 41.4 - 106.5 & 15.6 - 257.9 & 8.7 - 49.7 \\
% \hline
%\end{tabular}}
\caption{Quantitative error assessment on 3 U.S. states. We measure error on the testing period (Jan. 11 - Feb. 11, 2021) with respect to the observed counts at each possible care stage: general ward $\GG$, in ICU (including on and off ventilator) $\II + \VV$, on ventilator in ICU $\VV$, and \emph{smoothed} death counts $\XX$ sm.).
For all states and stages, we report the mean count $y$ across the testing period to give a sense of scale.
Cells marked NA were not available for that state (see discussion in App.~\ref{sec:app_datasets}).
AR-Poisson baseline is described in App.~\ref{sec:appendix_gar}, IHME baseline in App.~\ref{sec:appendix_ihme}.
We communicate uncertainty by reporting lower and upper estimates of the MAE.
To obtain these intervals for all variants of our ACED-HMM as well as our AR-Poisson baseline, we repeat all MAE computations across 100 separate batches of posterior samples.
We compute and report the 2.5th and 97.5th percentiles across these batches.
For the IHME baseline, a distribution of forecasted samples is not available.
Thus, we report the MAE computed using the mean estimate forecast, as well as the MAE computed using the provided lower and upper estimates count values.
This second kind of interval (marked with *) should not be directly compared to the first, as they capture different aspects of uncertainty.
}%endcaption
\label{tab:error_metrics_US}
\end{table}

